Learning Long Term Dependencies via Fourier Recurrent Units

It is a known fact that training recurrent neural networks for tasks that have long term dependencies is challenging. One of the main reasons is the vanishing or exploding gradient problem, which prevents gradient information from propagating to early layers. In this paper we propose a simple recurrent architecture, the Fourier Recurrent Unit (FRU), that stabilizes the gradients that arise in its training while giving us stronger expressive power. Specifically, FRU summarizes the hidden states $h^{(t)}$ along the temporal dimension with Fourier basis functions. This allows gradients to easily reach any layer due to FRU's residual learning structure and the global support of trigonometric functions. We show that FRU has gradient lower and upper bounds independent of temporal dimension. We also show the strong expressivity of sparse Fourier basis, from which FRU obtains its strong expressive power. Our experimental study also demonstrates that with fewer parameters the proposed architecture outperforms other recurrent architectures on many tasks.

==> my_vagrad.tex <==
\section{Vanishing and exploding gradient}\label{sec:vangrad}
In this section, we analyze the vanishing/exploding gradient issue in various
recurrent architectures. Specifically we give the lower/upper bound of 
gradient magnitude under linear setting and showed that gradient of FRU does 
not explode nor vanish with temporal dimension $T \rightarrow \infty$.
For simplicity, we consider the linear activation case where activations are identity 
mapping. We first analyze RNN and SRU models as a baseline and counter examples.
\paragraph{Gradient of linear RNN}
For RNN, we have:
\begin{align*}
  h^{(t+1)} = W \cdot h^{(t)} + U \cdot x^{(t)} + b
\end{align*}
where $t=0,1,2\cdots T-1$. Thus
\begin{align*}
  h^{(T)} = & ~ W \cdot h^{(T-1)} + U \cdot x^{(T-1)} + b \\
%  = & ~ W \cdot ( W \cdot h_{T-2} + U \cdot x_{T-2} + b ) \\
%  & ~ + U \cdot x_{T-1} + b \\
%  = & ~ W^2 \cdot h_{T-2} + W ( U \cdot x_{T-2} + b ) \\
%  & ~ + U \cdot x_{T-1} + b \\
%  = & ~ \cdots \\
  = & ~ W^{T-T_0} \cdot h^{(T_0)} + \sum_{t=T_0}^{T} W^{T-t-1} (U \cdot x^{(t)} + b)
\end{align*} 
Let $L = L(h^{(T)})$ denote the loss function. By Chain rule,
%\begin{align*}
%\frac{\partial L}{ \partial T_0} = \left( \frac{ \partial h_T }{\partial h_{T_0}} \right)^\top \frac{\partial L}{\partial h_T}
%\end{align*}
we have
\begin{align*}
  \left\| \frac{\partial L}{\partial h^{(T_0)} } \right\| = & ~ \left\| \left( 
    \frac{ \partial h^{(T)} }{\partial h^{(T_0)}} \right)^\top \frac{\partial 
  L}{\partial h^{(T)}} \right\|  \\
  = & ~ \left\| (W^{T-T_0})^\top \cdot \frac{\partial L}{\partial h^{(T)} } \right\| \\
  \geq & ~ \sigma_{\min} ( W^{T-T_0}  ) \cdot \left\| \frac{\partial L}{\partial h^{(T)} } \right\|.
\end{align*}
Similarly for the upper bound:
\begin{align*}
  \left\| \frac{\partial L}{\partial h^{(T_0)} } \right\| \leq & ~ \sigma_{\max} ( W^{T-T_0}  ) \cdot \left\| \frac{\partial L}{\partial h^{(T)} } \right\|.
\end{align*}

\paragraph{Gradient of linear SRU}
For SRU, we have:
\begin{align*}
  h^{(t)} = & ~ W_1W_2 \cdot u^{(t-1)} + W_2b_1 + W_3 \cdot x^{(t-1)} +b_2,\\
  u^{(t)} = & ~ \alpha \cdot u^{(t-1)} + (1-\alpha) h^{(t)}.
\end{align*}
Denote $W = W_1 W_2$ and $B = W_2 b_1 + b_2$, we have
%%% This is Claim
\define{cla:sru_ut_is_sum}{Claim}{
Let $\ov{W}=\alpha I + (1-\alpha) W$. Then using SRU update rule, we have
  $u^{(T)} =  \ov{W}^{T-T_0} u^{(T_0)}  + \sum_{t=T_0}^T \ov{W}^{T-t-1} (1-\alpha) W_3 (  x^{(t)} + B) $.
 }
\state{cla:sru_ut_is_sum}
We provide the proof in Appendix~\ref{app:vangrad}.

With $L=L(u^{(T)})$, by Chain rule, we have lower bound:
\begin{align*}
  \left\| \frac{\partial L}{\partial u^{(T_0)} } \right\| = & ~ \left\|  ( (\alpha I + (1-\alpha)W)^\top )^{T-T_0} \frac{\partial L}{\partial u^{(T)}} \right\| \\
  \geq & ~ (\alpha + (1-\alpha)\sigma_{\min}(W))^{T-T_0}  \cdot \left\| \frac{\partial L}{\partial u^{(T)}} \right\|.
\end{align*}
And similarly for upper bound:
\begin{align*}
  \left\| \frac{\partial L}{\partial u^{(T_0)} } \right\| \leq & ~ (\alpha  + (1-\alpha)\sigma_{\max}(W))^{(T-T_0)}  \cdot \left\| \frac{\partial L}{\partial u^{(T)}} \right\|.
\end{align*}
These bounds for RNN and SRU are achievable, a simple example would be 
$W=\sigma I$. 
Easy to notice that with $\alpha\in(0,1)$, SRU do have better gradient bounds 
than RNN. However, SRU is only better by a constant factor on the exponent and 
both method's gradient could still explode or vanish 
exponentially with temporal dimension $T$. 


\paragraph{Gradient of linear FRU}
By design, FRU avoided vanishing/exploding gradient by its residual learning 
structure. Specifically, linear \rm{FRU} has bounded gradient which is independent of the temporal 
dimension $T$. We have the following theorem:

\define{cla:fru_ut_is_sum}{Claim}{
$
u^{(T)} = \prod_{t=T_0+1}^T ( I + \frac{1}{T} \cos(2\pi f t/T + \theta)  W) u^{(T_0)} + \frac{1}{T} \sum_{t=T_0+1}^T \cos(2\pi f t / T + \theta) (W_3 x^{(t-1)} + B ).
$
}

\define{cla:fru_upper_bound_gradient}{Claim}{
\begin{align*}
\left\| \frac{\partial L}{ \partial u^{(T_0)} } \right\| \leq e^{ \sigma_{\max} (W) } \left\| \frac{\partial L}{\partial u^{(T)} } \right\|.
\end{align*}
}

\begin{theorem}
  With FRU update rule in \eqref{eq:fru_update_rule}, and $\phi$ being identity, we have: {\small
\begin{align*}
e^{- 2\sigma_{\max}(W_1W_2)} \left\| \frac{\partial L}{\partial u^{(T)}} \right\|
\leq \left\| \frac{\partial L}{ \partial u^{(T_0)} } \right\| \leq e^{ \sigma_{\max} (W_1W_2) } \left\| \frac{\partial L}{\partial u^{(T)}} \right\|
\end{align*}}
for any $T_0\leq T$.
\end{theorem}

\begin{proof}
For FRU, we have:
\begin{align}
  h^{(t)} = & ~ W_1 W_2 \cdot u^{(t-1)} + W_2b_1 + W_3 x^{(t-1)} +b_2, \notag \\
  u^{(t)} = & ~  u^{(t-1)} + \frac{1}{T} \cos( 2\pi ft/T + \theta) h^{(t)}. \notag 
\end{align}
Let $W = W_1 W_2$ and $B = W_2 b_1 + b_2$, we can rewrite $u^{(T)}$ in the following way,
%%% This is a Claim
\state{cla:fru_ut_is_sum}
We provide the proof of Claim~\ref{cla:fru_ut_is_sum} in Appendix~\ref{app:vangrad}. By Chain rule{\small
\begin{align*}
  \left\| \frac{\partial L}{\partial u^{(T_0)}} \right\|= & ~ \left\| \left( \frac{\partial h^{(T)}}{\partial h^{(T_0)}} \right)^\top \frac{\partial L}{\partial h^{(T)}} \right\| \\
  = & ~ \left\| \left(\prod_{t=T_0+1}^T (I + \frac{1}{T} \cos ( 2\pi f t /T + \theta ) \cdot W ) \right)^\top \frac{\partial L}{\partial u^{(T)}} \right\| \\
  \geq & ~ \sigma_{\min} \left( \prod_{t=T_0+1}^T (I + \frac{1}{T} \cos ( 2\pi f t /T + \theta ) \cdot W ) \right) \cdot \left\| \frac{\partial L}{\partial u^{(T)}} \right\| \\
  \geq & ~   \prod_{t=T_0+1}^T \sigma_{\min} (I + \frac{1}{T} \cos ( 2\pi f t /T + \theta ) \cdot W ) \cdot \left\| \frac{\partial L}{\partial u^{(T)}} \right\|
\end{align*}}
We define two sets $S_-$ and $S_+$ as follows {\small
\begin{align*}
S_- = \{ t ~|~ \cos (2\pi f t /T + \theta) < 0, t = T_0+1, T_0+2, \cdots, T \} \\
S_+ = \{ t ~|~ \cos (2\pi f t /T + \theta) \geq 0, t = T_0+1, T_0+2, \cdots, T \}
\end{align*}}
Thus, we have
\begin{align*}
  & ~ \prod_{t=T_0+1}^T \sigma_{\min} (I + \frac{1}{T} \cos ( 2\pi f t /T + \theta ) \cdot W ) \\
 = & ~ \prod_{t \in S_+} (1 + \frac{1}{T} \cos ( 2\pi f t /T + \theta ) \cdot \sigma_{\min} (W) ) \\
 & ~ \cdot \prod_{t \in S_-} (1 + \frac{1}{T} \cos ( 2\pi f t /T + \theta ) \cdot \sigma_{\max} (W) )
\end{align*}
The first term can be lower bounded by $1$ easily, the next question is how to lower bound the second term. Since $\sigma_{\max} < T$, we can use the fact $1 - x \geq e^{-2x}, \forall x \in [0,1]$,
\begin{align*}
& ~\prod_{t \in S_-} (1 + \frac{1}{T} \cos ( 2\pi f t /T + \theta) \cdot \sigma_{\max} (W) ) \\
 \geq & ~ \prod_{t \in S_-} \exp( -2 \frac{1}{T} |\cos(2\pi f t/T + \theta)| \sigma_{\max}(W) ) \\
 = & ~ \exp \left( -2 \sum_{t \in S_-} \frac{1}{T} |\cos(2\pi f t/T + \theta)| \sigma_{\max}(W) \right) \\
 \geq & ~ \exp(- 2\sigma_{\max}(W))
\end{align*}
where the last step follows by $|S_-| \leq T$ and $|\cos(2\pi f t/T + \theta)| \leq 1$. 

Therefore, we complete the proof of lower bound.


Similarly, we can show the upper bound
\state{cla:fru_upper_bound_gradient}
We provide the proof in Appendix~\ref{app:vangrad}. Combining the lower bound and upper bound together, we complete the proof.
\end{proof}



==> preli.tex <==
%\section{Preliminaries}\label{sec:preli}







